Galaxy Cluster Statistics in Modified Gravity Cosmologies

If the accelerated expansion of the universe is due to a modification of general relativity at late times, it is likely that the growth of structure on large scales would also display deviations from the standard cosmology. We investigate the statistics of the distribution of galaxy cluster-sized halos as a probe of gravity. We analyze the output of several matched N-body simulations with the same initial conditions and expansion histories but using both DGP and f (R) gravity with various parameters. From each simulation we extract the cluster mass function, power spectrum, and mean pairwise velocity at redshifts 1, 0.3, and 0. All three statistics display systematic differences between gravity theories. The mean pairwise velocity provides an important consistency test for any posited departure from general relativity suggested by measurements of the power spectrum and cluster mass function. Upcoming microwave background experiments, including Simons Observatory and CMB- S4, will detect tens of thousands of galaxy clusters via the thermal Sunyaev-Zeldovich effect, probe their masses with lensing of the microwave background, and potentially measure velocities using the transverse lensing effect or the kinematic Sunyaev-Zeldovich effect. These cluster measurements promise to be a substantial probe of modified gravity.

==> bibliography.tex <==
\begin{thebibliography}{}

\bibitem{Abbott17.2}
Abbott, B. P. Centennial of General Relativity, 5 Feb. 2017, pp. 291–311, 10.1142/9789814699662\_0011.

\bibitem{Abbott17.8}
Abbott, B. P., et al. The Astrophysical Journal, vol. 848, no. 2, 16 Oct. 2017, p. L13, doi:10.3847/2041-8213/aa920c.

\bibitem{Planck15}
Ade, P. A. R., et al. Astronomy \& Astrophysics, vol. 594, 20 Sept. 2016, p. A27, 10.1051/0004-6361/201525823. 

\bibitem{SO19}
Ade, P., et al. Journal of Cosmology and Astroparticle Physics, vol. 2019, no. 02, 27 Feb. 2019, pp. 056–056, 10.1088/1475-7516/2019/02/056.

\bibitem{Alam21}
Alam, S., et al. Journal of Cosmology and Astroparticle Physics, vol. 2021, no. 11, 1 Nov. 2021, p. 050, 10.1088/1475-7516/2021/11/050. 

\bibitem{Baker13}
Baker, T., et al. Physical Review D, vol. 87, no. 2, 7 Jan. 2013, 10.1103/physrevd.87.024015.

\bibitem{Barreira15}
Barreira, A., et al. Journal of Cosmology and Astroparticle Physics, vol. 2015, no. 12, 30 Dec. 2015, pp. 059–059, 10.1088/1475-7516/2015/12/059.

\bibitem{Behroozi12}
Behroozi, P. S., Wechsler, R. H., \&; Wu, H., The Astrophysical Journal, 762(2), 109 (2012), doi:10.1088/0004-637x/762/2/109.

\bibitem{Bernardis17}
Bernardis, F. D., et al.,  Journal of Cosmology and Astroparticle Physics, 2017(03), 008-008 doi:10.1088/1475-7516/2017/03/008.

\bibitem{Bhattacharya08}
Bhattacharya, S. \&; Kosowsky, A. Physical Review D, vol. 77, no. 8, 24 Apr. 2008, 10.1103/physrevd.77.083004.

\bibitem{Blas11}
Blas, D., et al. Journal of Cosmology and Astroparticle Physics, vol. 2011, no. 07, 22 July 2011, pp. 034–034, 10.1088/1475-7516/2011/07/034.

\bibitem{Bleem20}
Bleem, L. E., et al. The Astrophysical Journal Supplement Series, vol. 247, no. 1, 5 Mar. 2020, p. 25, 10.3847/1538-4365/ab6993.

\bibitem{Cautun18}
Cautun, M., et al. Monthly Notices of the Royal Astronomical Society, vol. 476, no. 3, 22 Feb. 2018, pp. 3195–3217, 10.1093/mnras/sty463.

\bibitem{Dvali00}
Dvali, G., Gabadadze, G., \&; Porrati, M., Physics Letters B, 484(1-2), 112-118 (200). doi:10.1016/s0370-2693(00)00631-6.

\bibitem{Gong18}
Gong, Y., Papantonopoulos, E., \&; Yi, Z., The European Physical Journal C, 78(9) (2018), doi:10.1140/epjc/s10052-018-6227-9.

\bibitem{Hand}
Hand, N., et al. The Astronomical Journal, vol. 156, no. 4, 18 Sept. 2018, p. 160, 10.3847/1538-3881/aadae0.

\bibitem{Hernandez18}
Hernández-Aguayo, C., et al. Monthly Notices of the Royal Astronomical Society, vol. 479, no. 4, 7 July 2018, pp. 4824–4835, 10.1093/mnras/sty1822.

\bibitem{Hilton21}
Hilton, M., et al. The Astrophysical Journal Supplement Series, vol. 253, no. 1, 16 Feb. 2021, p. 3, 10.3847/1538-4365/abd023.

\bibitem{Hindshaw13}
Hinshaw, G., et al. The Astrophysical Journal Supplement Series, vol. 208, no. 2, 20 Sept. 2013, p. 19, 10.1088/0067-0049/208/2/19.

\bibitem{Hotinli21}
Hotinli, Selim C., et al. Physical Review D, vol. 104, no. 8, 19 Oct. 2021, 10.1103/physrevd.104.083529.

\bibitem{Hu07}
Hu, W., \& Sawicki I. Physical Review D, vol. 76, no. 6, 10 Sept. 2007, 10.1103/physrevd.76.064004. 

\bibitem{Langlois18}
Langlois, D., et al. Physical Review D, vol. 97, no. 6, 26 Mar. 2018, doi:10.1103/physrevd.97.061501.

\bibitem{Li12}
Li, B., et al. Journal of Cosmology and Astroparticle Physics, vol. 2012, no. 01, 27 Jan. 2012, pp. 051–051, 10.1088/1475-7516/2012/01/051.

\bibitem{Lombriser09}
Lombriser, L., et al. Physical Review D, vol. 80, no. 6, 28 Sept. 2009, 10.1103/physrevd.80.063536.

\bibitem{Lovelock71}
Lovelock, D., Journal of Mathematical Physics 12, no. 3 (1971): 498-501, doi:10.1063/1.1665613.

\bibitem{Shapiro71}
Shapiro, I., Nature Physical Science 231, no. 20 (1971): 48. doi:10.1038/physci231048a0.

\bibitem{Stein20}
Stein, G., et al. Journal of Cosmology and Astroparticle Physics, vol. 2020, no. 10, 5 Oct. 2020, pp. 012–012, 10.1088/1475-7516/2020/10/012.

\bibitem{Sunyaev72}
Sunyaev R. A. \&; Zeldovich Y. B., Comments on Astrophysics and Space Physics 4, 173 (1972).

\bibitem{Teyssier02}
Teyssier, R. Astronomy \& Astrophysics, vol. 385, no. 1, Apr. 2002, pp. 337–364, 10.1051/0004-6361:20011817.

\bibitem{Vikram13}
Vikram, V., et al. Journal of Cosmology and Astroparticle Physics, vol. 2013, no. 08, 9 Aug. 2013, pp. 020–020, 10.1088/1475-7516/2013/08/020.

\bibitem{Will14}
Will, C. M. Living Reviews in Relativity 17, no. 1 (2014). doi:10.12942/lrr-2014-4.


\end{thebibliography}


%begin{center}
%	\begin{table}%[ht]
%	    \begin{tabular}{|c|c|c|c|}
%	        \hline
%		    \multicolumn{4}{|c|}{$v_{ij}^{GR}(r) - v_{ij}^{MG}(r)$ (km/s)}\\
%		    \hline
%		   (Mpc) & $0 < r < 10$ & $10 < r < 20$ & $20 < r < 30$ \\
%		    \hline
%		    F4 & 117.80 $\pm$ 53.18 & 37.95 $\pm$ 30.35 & 33.08 $\pm$ 27.90\\
%		    \hline
%		    F5 & -15.63 $\pm$ 60.11 & 25.97 $\pm$ 33.76 & -21.61 $\pm$ 30.95\\
%		    \hline
%		    F6 & 11.40 $\pm$ 59.49 & 42.61 $\pm$ 33.88 & -12.96 $\pm$ 31.43\\
%		    \hline
%		    N1 & 58.58 $\pm$ 54.61 & 47.66 $\pm$ 32.52 & -74.95 $\pm$ 29.26\\
%		    \hline
%		    N5 & 25.50 $\pm$ 54.61  & 55.06 $\pm$ 33.74  & -22.39 $\pm$ 31.32\\
%		    \hline
%	    \end{tabular}
%	    \quad
%	    \begin{tabular}{|c|c|c|c|}
%	        \hline
%		    \multicolumn{4}{|c|}{$v_{ij}^{GR}(r) - v_{ij}^{MG}(r)$ (km/s)}\\
%		    \hline
%		   (Mpc) & $0 < r < 10$ & $10 < r < 20$ & $20 < r < 30$ \\
%		    \hline
%		    F4 & 120.66 $\pm$ 17.33 & 71.11 $\pm$ 8.88 & 17.91 $\pm$ 6.96\\
%		    \hline
%		    F5 & 0.36 $\pm$ 16.40 & -0.86 $\pm$ 8.67 & -18.78 $\pm$ 6.92\\
%		    \hline
%		    F6 & -0.76 $\pm$ 17.26 & 7.36 $\pm$ 9.13 & -7.40 $\pm$ 7.26\\
%		    \hline
%		    N1 & 77.60 $\pm$ 16.54 & 65.27 $\pm$ 8.92 & 30.79 $\pm$ 7.10\\
%		    \hline
%		    N5 & 21.95 $\pm$ 16.89 & 23.31 $\pm$ 9.03 & 3.25 $\pm$ 7.27\\
%		    \hline
%	    \end{tabular}
%	    \quad
%	    \begin{tabular}{|c|c|c|c|}
%	        \hline
%		    \multicolumn{4}{|c|}{$v_{ij}^{GR}(r) - v_{ij}^{MG}(r)$ (km/s)}\\
%		    \hline
%		   (Mpc) & $0 < r < 10$ & $10 < r < 20$ & $20 < r < 30$ \\
%		    \hline
%		    F4 & 116.82 $\pm$ 13.23 & 58.85 $\pm$ 6.83 & 21.54 $\pm$ 4.98\\
%		    \hline
%		    F5 & 4.43 $\pm$ 12.15 & -1.48 $\pm$ 6.58 & -1.42 $\pm$ 4.81\\
%		    \hline
%		    F6 & -1.56 $\pm$ 12.87 & 6.60 $\pm$ 6.96 & -2.79 $\pm$ 5.12\\
%		    \hline
%		    N1 & 45.00 $\pm$ 13.21 & 47.05 $\pm$ 6.93 & 30.11 $\pm$ 5.11\\
%		    \hline
%%		    \hline
%	    \end{tabular}
%	    \caption{In order of \emph{decreasing} redshift, these tables show the difference between the MPV as calculated with GR halos and the MPV of each MG model and the quadrature error. We print the first three separation bins as a means of comparison because this is the regime where differences can be most precisely %measured.}
%	    \label{tab:mpv_table}
%	\end{table}
%\end{center}

%\begin{center}
%	\begin{table}%[ht]
%	    \centering
%	    \begin{tabular}{|c|c|c|c|}
%	        \hline
%		    \multicolumn{4}{|c|}{$\chi^2$}\\
%		    \hline
%		    & $z = 1.0$ & $z = 0.3$ & $z = 0$ \\
%		    \hline
%		    F4 & 37.77 & 312.03 & 552.54\\
%		    \hline
%		    F5 & 7.42 & 113.37 & 135.66\\
%		    \hline
%		    F6 & 11.47 & 7.47 & 21.56\\
%		    \hline
%		    N1 & 44.12 & 716.00 & 1284.75\\
%		    \hline
%		    N5 & 15.88 & 38.89 & 303.41\\
%		    \hline
%	    \end{tabular}
%	    \caption{Table of $\chi^2$ values for the mean pairwise velocity for each modified gravity model where we treat the MPV $\pm$ some error correction for GR as our "data" and the modified gravity theories as our "models" to fit our data. We took the error of the points to be the standard error we computed from the MPV that we referenced earlier.}
%	    \label{tab:chi_tab}
%	\end{table}
%\end{center}
